Carnap: An Open Framework for Formal Reasoning in the Browser

This paper presents an overview of Carnap, a free and open framework for the development of formal reasoning applications. Carnap's design emphasizes flexibility, extensibility, and rapid prototyping. Carnap-based applications are written in Haskell, but can be compiled to JavaScript to run in standard web browsers. This combination of features makes Carnap ideally suited for educational applications, where ease-of-use is crucial for students and adaptability to different teaching strategies and classroom needs is crucial for instructors. The paper describes Carnap's implementation, along with its current and projected pedagogical applications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{70}
\providecommand{\publicationstatus}{P. Quaresma and W. Neuper (Eds.): 6th International Workshop\\ on Theorem proving components for Educational software (ThEdu'17)\\
EPTCS 267, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.267.5}{10.4204/EPTCS.267.5}}
\pdfoutput=1

